Breaking Type Safety in Go: An Empirical Study on the Usage of the unsafe Package

A decade after its first release, the Go programming language has become a major programming language in the development landscape. While praised for its clean syntax and C-like performance, Go also contains a strong static type-system that prevents arbitrary type casting and arbitrary memory access, making the language type-safe by design. However, to give developers the possibility of implementing low-level code, Go ships with a special package called unsafe that offers developers a way around the type-safety of Go programs. The package gives greater flexibility to developers but comes at a higher risk of runtime errors, chances of non-portability, and the loss of compatibility guarantees for future versions of Go. In this paper, we present the first large-scale study on the usage of the unsafe package in 2,438 popular Go projects. Our investigation shows that unsafe is used in 24% of Go projects, motivated primarily by communicating with operating systems and C code, but is also commonly used as a source of performance optimization. Developers are willing to use unsafe to break language specifications (e.g., string immutability) for better performance and 6% of analyzed projects that use unsafe perform risky pointer conversions that can lead to program crashes and unexpected behavior. Furthermore, we report a series of real issues faced by projects that use unsafe, from crashing errors and non-deterministic behavior to having their deployment restricted from certain popular environments. Our findings can be used to understand how and why developers break type-safety in Go, and help motivate further tools and language development that could make the usage of unsafe in Go even safer.

==> Discussion_Dependency.tex <==

As discussed in \Cref{sub:backgrond-risk-unsafe}, using the \unsafe package breaks the guarantee of compatibility promised at the first version of Golang.
We investigate how many packages and projects would be affected if a breaking change in \unsafe were introduced at the next version of Go.
In the past, changes in hte \unsafe package had caused some programs to stopped working~\tocite{bugs}, and two proposals for Go 2.0 (the next major milestone for the languauge)~\cite{proposal:unsafe1:online,proposal:unsafe2:online} contain language changes in \unsafe that have the potential for breaking programs that use \unsafe today.  

Motivated by this uncertainty, we expore a worst-case scenario of the impact of a future change in the \unsafe package. 
We consider a project affected if 1) the project uses \unsafe, regardless of the function used, or 2) the project depends on external packages that use \unsafe, regardless of whether the function that calls \unsafe is called by the project.
Having a grasp on the impact of \unsafe changes in the most popular Go projects might help inform the Go community and the language maintainers on how to better plan future changes to \unsafe to mitigate the impact in Go projects.


In our dataset of \datasetsize projects, we have approximately 60 thousand packages.
We list the dependencies of each package through the \code{go list}~\cite{Go:list:online} command, which exports exports all direct dependencies of all packages identified in all sub-directories in a project. 
Similarly to our methodology presented in \Cref{sub:rq_usage}, we exclude the results from vendor folders. 
We use direct dependencies to build a package dependency graph, and analyze this graph to identify packages that depend on other packages that use \unsafe.


\diego{Add the results and a brief discussion over the Go dependency network.}





\begin{table}
	\caption{Number of projects possibly affected by any breaking change in \unsafe}
	\label{tab:rq2-affected-dependencies}
	\include{tables/rq2-affected-dependencies}
\end{table}

==> Discussion_usagepatterns.tex <==


In this section, we will explore in depth some of the findings obtained in the manual analysis.

\textbf{Commonly used type conversion code.}

\begin{itemize}
	\item Discuss the cases where the same file \textit{zz\_generated.conversion.go} is used across multiple projects. 
	\item How many projects contain this particular file?
\end{itemize}




==> PreliminaryAnalysis.tex <==

This section will serve as a report of the initial phases of the project. 
Later, this section shall be broken into multiple sections, involving methodology, results and discussion. 

In this preliminary analysis, we are focusing on answering the following research questions:

\begin{enumerate}
	\item[RQ1] Is \unsafe used in open-source Go projects?
	\item[RQ2] How often does a Go project depend on packages that use \unsafe?
	\item[RQ3] Do developers follow the good practices of \unsafe documentation?
	\item[RQ4] Does the use of \unsafe change over time?
	
	
\end{enumerate}

\subsection{Data Selection}

To investigate the aforementioned research questions, we clone the most popular go projects from GitHub.
We first query the GitHub Request API to identify the top 3,060 most starred Go repositories, as the number of stars is a good indicator of the project popularity within GitHub repositories.

Even among the most popular projects we may find abandoned repositories.
As we want to evaluate the usage of \unsafe on active projects, in particular when measuring the effects of compatibility breaks in future versions of Go, we further curate our dataset by removing projects that have not pushed any contribution for the last 12 months (September 2018).
This process yields a dataset composed of 2,590 go projects (see \Cref{tab:dataset}).

\begin{table}
	\caption{Composing the dataset for this investigation. 
		We considered inactive projects, repositories that have not pushed any contribution in the last 12 months.}
	\label{tab:dataset}
	\input{tables/dataset}
\end{table}



\begin{figure}
	\includegraphics[width=\linewidth]{figures/dataset-stars}
	\caption{Distribution of projects' stars count of our dataset. Note the log scale on the x axis.}
	\label{fig:dataset-stars}
\end{figure}

\begin{figure}
	\includegraphics[width=\linewidth]{figures/dataset-age-months}
	\caption{Distribution of projects' age in months of our dataset.}
	\label{fig:dataset-age-months}
\end{figure}



\subsection{RQ1. Is \unsafe used in open-source Go projects?}

\textbf{Motivation.} 



\textbf{Approach.}
To find whether projects make use of \unsafe in their source-code, we build a parser for Golang, using the support of Go's native \code{ast} package~\footnote{https://golang.org/pkg/go/ast/}.
Our parser inspects the AST of the parsed go file and identifies the function calls and type references to the \unsafe package.
We run this parser in every go file present in our dataset of repositories, but filter out usages identified in the source-code of the project dependencies.
Until recently, a common practice in Go projects for managing dependencies was to include all dependencies in the projects structure, in a folder called "vendor". 
Hence, we exclude all reports of \unsafe usage originating from vendor folders.


\textbf{Results.}
In \Cref{tab:rq1:descriptive} we show that from the 2590 evaluated repositories, \textbf{618 (23.8\%) make use of \unsafe directly in the project source-code}. 
The extent in which projects use \unsafe varies considerably, as shown in~\Cref{fig:rq1-distribution-projects}, the majority of projects (74\%) use \unsafe sparsely in their code, with less than 100 calls to \unsafe operations.
Yet, 77 projects in ou our dataset rely heavily at \unsafe to program their routines, with more than 100 operations present in their source-code.

The \unsafe API is very compact, composed of only one type definition (\code{Pointer}) and three exported functions (\code{SizeOf())}, \code{OffsetOf()}, \code{AlignOf()}). 
The vast majority of \unsafe operations used by open-source Go projects is concentrated in the \code{unsafe.Pointer} type (\Cref{tab:rq1-most-used-features}).
The functions are used less frequently and represent together just 2.23\% of used \unsafe operations.

\diego{Update with the latest results}
We present the top-10 projects with the highest reliance on \unsafe in \Cref{tab:rq1-top10-projects}.
Among the top-10, four projects are a framework for the cross-platform Qt\footnote{https://www.qt.io}, an open-source widget toolkit for creating graphical interfaces. 
These projects provide bindings from Qt to a myriad of platforms, and need to work with low-level routines to accomplish such portability.
Overall, seven out of the top-10 projects deal with bindings to or from graphical interfaces: 4 from Qt, one binding to OpenGL, one widgets wrapper and a visual web-server. 
\diego{Add here some more comments on why graphical interface application would need the flexibility of \unsafe}

The Golang project itself makes an extensive use of \unsafe for implementing low-level routines. 
While discouraged by the official documentation and community, if used correctly \unsafe can be properly applied to \diego{Add here where \unsafe is mostly used in golang.}


\begin{table}
	\caption{Descriptive statistics on the projects that use \unsafe. Our dataset is comprised by  }
	\label{tab:rq1:descriptive}
	\include{tables/rq1-descriptive}
\end{table}

\begin{figure}
	\includegraphics[width=\linewidth]{figures/rq1-projects-dist}
	\caption{Distribution of projects that make use of \unsafe by the number of \unsafe operation calls}
	\label{fig:rq1-distribution-projects}
\end{figure}

\begin{table}
	\caption{\unsafe operations ranked by their usage.}
	\label{tab:rq1-most-used-features}
	\include{tables/rq1-most-used-features}
\end{table}

\begin{figure}
	\includegraphics[width=\linewidth]{figures/rq1-projects-dist-operation}
	\caption{Distribution of \unsafe opertions in the 618 projects that use unsafe.}
	\label{fig:rq1-ditribution-projects-operations}
\end{figure}


\begin{table}
	\caption{Top 10 projects with highest number of \unsafe method calls}
	\label{tab:rq1-top10-projects}
	\include{tables/rq1-projects}
\end{table}


\subsection{RQ2. How often does a project depend on packages that uses \unsafe?}

\textbf{Motivation.} Packages that use \unsafe are not guaranteed to be compatible with future versions of Go. 
Golang maintainers reserve the right to update internal structures of the language that may impact how \unsafe is implemented, hence, introducing breaking changes in future versions of the language.
In this question, we focus on investigating how many packages and projects would be affected if a breaking change is introduced in \unsafe.
Answering this question may shed a light on the impact of future Go version in the ecosystem and inform language maintainers on how to better plan future changes to \unsafe to mitigate the impact in Go projects.

\textbf{Approach.}
In Go, packages (libraries) are the reusable units among software projects. 
Project dependencies are established by installing and importing third-party packages from the Go ecossystem.
One Go project may export dozens of reusable packages, and each package commonly reutilizes a handful of other packages from the same project (internal dependencies) and from external applications (external dependencies).
Hence, to understand the spread of \unsafe usafe within Go application dependencies, we need to analyse this question at the package level.

In our dataset of 3k projects, we have a total of \todo{X} packages.
We list the dependencies of each package through the following native go command:

\code{go list -f "\{\{.ImportPath\}\}, \{\{.Imports\}\}" ./...}


This command exports all direct dependencies of all packages identified in all sub-directories in a project. 
We use direct dependencies to build a package dependency graph, and analyze this graph to identify packages that depend on other packages that use \unsafe.
We group this analysis per project, and consider a project \textit{dependent} of an \unsafe package, if at least one of its own packages depend on a package that uses \unsafe.
Furthermore, we also analyze the transitive dependencies of all packages in a project, that is, the dependencies of the dependencies of a project's packages (one level of indirection).
If a project has a transitive dependency that uses \unsafe, we categorize the project as being \textit{transitively-dependent} of an \unsafe package.

\diego{Add here a brief data analysis of the dependency graph: how many nodes, edges? Is the network highly connected? This could also go to the Discussion section.}


\textbf{Results.}
\todo{TBD}



\begin{figure}
	\includegraphics[trim={0 4cm 0 4cm}, clip, width=\linewidth]{figures/dependency-graph-affected-straight}
	\caption{Dependency graph showing only the dependencies to projects that use \unsafe (24.5\% of the original graph edges).}
	\label{fig:dependency-graph-affected}
\end{figure}

\begin{table}
	\caption{Number of projects possibly affected by any breaking change in \unsafe}
	\label{tab:rq2-affected-dependencies}
	\include{tables/rq2-affected-dependencies}
\end{table}

\subsection{RQ3. Do developers follow the good practices of \unsafe documentation?}

\textbf{Motivation.}
Using \unsafe operations is not necessarily a bad smell in the code.
The official documentation of \unsafe describes at length how to safely use \unsafe , by showing valid usage patterns and describing some of the pitfalls developers must avoid.
In this question, we explore if developers follow the recommendations of \unsafe documentation and help identify scenarios in which the code is not guaranteed to behave as intended.
Answering this question will help us understand the typical mistakes developers make, and contribute to devise better tools to assist developers at using \unsafe properly.

\textbf{Approach.}
Finding valid bad practices in the code is a difficult task.
Static analyzers are very useful to pinpoint bad practices and are used on a daily based by developers, but are prone to false reports and cannot guarantee recall (i.e., that the reports cover all issues in the code) in every scenario.
For this preliminary analysis, we focus on a particular pattern of misuse: \textbf{conversion of \code{uintptr} to \code{unsafe.Pointer}}, as this pattern is well-documented and covered by a native go code analyser: go vet~\cite{vetTheGo72:online}.
The command vet examines Go source-code to report suspicious statements under a variety of bad practices, and covers the aforementioned bad practice related to \unsafe.

To analyse the projects that use \unsafe with \code{go vet}, we use Go Report Card~\cite{schaaf-smith-goreportcard} web platform, which generates reports under a variety of code analysers.
To run this analyzer, we need to automatically compile the projects in our dataset.
As shown in previous studies~\todo{Add refs}, building hundreds of project is a challenging task as some projects require specific dependencies, environments or may not be suitable for independent automatically builts.
From the original set of 701 projects that use \code{unsafe}, we could automatically build and analyze 489 projects.


\textbf{Caveat/Threat to validity.}
The results presented in the preliminary analysis are based on reports generated from Go Report Card that are from 2 months to 1 year old.
Some of these reports may have been already fixed and some new cases may appear in the newest version of the projects' source-code.
This is far from ideal and should be addressed in the final version of this project.

I have tried to semi-manually update the reports, but I found a bug in the original code: the current version of \texttt{go vet}  is not working with the online version of Go Report Card. 
I have issued a bug report~\footnote{https://github.com/gojp/goreportcard/issues/300} but could also later re-generate the reports locally, as my local version of Go Report Card seems to be working properly.

\textbf{Results.}
We present the overview of the results in~\Cref{tab:rq3-reports}.
From the set of 489 projects analyzed, \textbf{52 projects (10\%) were flagged with suspicious \code{unsafe.Pointer} usage.}
Most projects, however, have less than 20 cases of invalid conversions of \code{uintptr} to \code{unsafe.Pointer} (\Cref{fig:rq3-projects-dist}). 

In~\Cref{tab:rq3-top10-unsafe-badpractices} we report the 10 projects with the highest number of reported  misues of \unsafe.
We observe five projects with more than 100 cases of invalid conversion from \code{uintptr} to \code{unsafe.Pointer}, including sqlite with a surprising 6496 reports in their source-code.
\diego{We need to analyse this projects in details and explain here why such projects have such a high number of potential invalid conversions.}


\begin{table}
	\caption{Number of projects with at least one occurrence of suspicious \code{unsafe} usage}
	\label{tab:rq3-reports}
	\include{tables/rq3-reports}
\end{table}

\begin{figure}
	\includegraphics[width=\linewidth]{figures/rq3-projects-dist}
	\caption{Distribution of reported suspicious \code{unsafe.Pointer} }
	\label{fig:rq3-projects-dist}
\end{figure}

\begin{table}
	\caption{Top 10 projects with the highest number of reported suspicious \code{unsafe.Pointer} usage}
	\label{tab:rq3-top10-unsafe-badpractices}
	\include{tables/rq3-top10-unsafe-badpractices}
\end{table}

\subsection{RQ4. Does the use of \unsafe change over time?}

\textbf{Motivation.}

\textbf{Approach.}

\textbf{Results.}




==> RQ_TrendUsage.tex <==

\noindent\textbf{Motivation:}

\noindent\textbf{Approach:}

\noindent\textbf{Results:}


\conclusion{}

==> Results.tex <==



\subsection{RQ1. \rqone}
\label{sub:rq_usage}
\input{RQ_Usage}

\subsection{RQ2. \rqtwo}
\label{sub:rq_usagepatterns}
\input{RQ_UsagePatterns}

\subsection{RQ3. \rqthree}
\label{sub:rq_badpractices}
\input{RQ_BadPractices}




==> rq2-usage-patterns.tex <==

\definecolor{bluegray}{rgb}{0.4, 0.6, 0.8}

\def\scale#1{%
	\numexpr#1 / 5\relax}

\def\mybar#1{%
	{\color{bluegray}\rule{\scale{#1}mm}{7pt}}} 

\begin{tabular}{l|l|ll}
	\toprule
	\textbf{Usage Patterns} & \textbf{Description}	& \textbf{Frequency}	&			\\
	\midrule
	
	\begin{minipage}{5cm}
		\renewcommand\DTstyle{\rmfamily}
		\dirtree{%
			.1 unsafe.
			.2 \textbf{Type/Array Casting}.
			.3 System Calls.
			.3 CGO.
			.3 Performance Optimization.
			.3 Reflection.
			.4 Marshaling.
			.3 Thread Synchronization.
			.2 \textbf{Memory Manipulation}.
			.3 Pointer Arithmetics.
			.2 \textbf{Size of Object}.
			.3 Getting Architecture Info.
			.2 \textbf{Unclear}.
			.2 \textbf{Others}.
		}
		
	\end{minipage}
	
	&
	
	\begin{minipage}{8cm}
		\renewcommand\DTstyle{\rmfamily} %
		\DTsetlength{0pt}{0pt}{0pt}{0pt}{0pt} %
		
		\dirtree{%
			.1 .
			.1 \textbf{Unsafe type/array casting using \unsafe}.
			.1 Using \unsafe to perform system calls.
			.1 Using \unsafe to communicate with C code via \cgo .
			.1 Bypassing type-checking and memory copy for performance.
			.1 Using the \texttt{reflect} to access object's metadata.
			.1 Using \unsafe with \texttt{reflect} to (de-)serialize json files.
			.1 Using \unsafe to write atomic operations with \texttt{atomic/sync}.
			.1 \textbf{Using \unsafe to get memory addresses and copy memory}.
			.1 Using \unsafe to perform pointer address arithmetics.
			.1 \textbf{Inspecting object size in memory}.
			.1 Inspecting the cpu architecture through \texttt{sizeOf(int)} method.
			.1 \textbf{Unclear usage-patterns}.
			.1 \textbf{Other use-cases (project specific)}.
		}
		
	\end{minipage}
	
	&
	
	\begin{minipage}{1.5cm}
		\renewcommand\DTstyle{\rmfamily} %
		\DTsetlength{0pt}{0pt}{0pt}{0pt}{0pt} %
		
		\begin{flushright} %
	
		\dirtree{%
			.0 .
			.0 \textbf{78.87\%}.
			.1 27.72\%.
			.1 17.98\%.
			.1 8.24\%.
			.1 7.12\%.
			.2 4.12\%.
			.1 3.37\%.
			 %
			.0 \textbf{3.37\%}.
			.1 2.25\%.
			.0 \textbf{6.74\%}. 
			.1 4.49\%.
			.0 \textbf{3.00\%}.
			.0 \textbf{8.24\%}. 
		}

		\end{flushright}

	\end{minipage}
	
	&
	
	\begin{minipage}{1.5cm}
		\renewcommand\DTstyle{\rmfamily} %
		\DTsetlength{0pt}{0pt}{0pt}{0pt}{0pt} %
		
			\dirtree{%
				.1 .
				.1 \mybar{78}.
				.1 \mybar{27}.
				.1 \mybar{17}.
				.1 \mybar{8}.
				.1 \mybar{7}.
				.1 \mybar{4}.
				.1 \mybar{3}.
				.1 \mybar{3}.
				.1 \mybar{3}.
				.1 \mybar{6}. 
				.1 \mybar{4}.
				.1 \mybar{3}.
				.1 \mybar{8}. 
			}
		
	\end{minipage}
	
	\\
	
	\bottomrule
\end{tabular}

==> tables/dataset.tex <==

\begin{tabular}{l|r}
	\toprule
	\textbf{Curation process} &     \textbf{\#} \\
	\midrule
	Initial dataset           			&  3,000 \\
	Remove forked projects & 0 \\
	Remove archived    			&    89  \\
	Remove inactive projects    &   371 \\
	Remove projects with less than 10 commits         &    22 \\
	Remove educational projects &    57 \\
	Clone errors 								& 24		\\
	\midrule
	\textbf{Total of projects}         				& \textbf{ 2,438}\\
	\bottomrule
\end{tabular}




==> tables/rq1-projects.tex <==
\begin{tabular}{llr}
	\toprule
	\textbf{Project}           & \textbf{Category} & \textbf{ \# of \unsafe} \\
	&			& operations \\
	\midrule
	therecipe/qt			 & Qt binding Framework		  & 42738 \\
	go-gl/gl           		  &  Go binding to OpenGL		&24930 \\
	kitech/qt.go 			& Qt binding Framework 		  & 24548 \\
	dontpanic92/wxGo & Widgets Wrapper				  & 13013 \\
	\textbf{golang/go}      & Programming Language 		&  8667 \\
	TeaWeb/build       		&  Visual Web Server 		& 8636 \\
	go-qml/qml         		& Qt binding Framework				&   8545 \\
	\textbf{golang/sys }   & Suplementary low-level library  & 8525 \\
	getlantern/lantern 		&  \todo{add} &5163 \\
	vulkan-go/vulkan   		& CG API binding   &4118 \\
	\bottomrule
\end{tabular}

==> tables/rq2-affected-dependencies.tex <==
\begin{tabular}{l|r|r}
\toprule
\textbf{\# of Projects affected by \unsafe} &     \textbf{\# }&     \textbf{\%} \\
\midrule
Affected directly                  &   701 & 23.56 \\
Affected only through direct dependency &   488 & 16.40 \\
Total affected                     &  1189 & 39.95 \\
\bottomrule
\end{tabular}

==> tables/rq3-reports.tex <==
\begin{tabular}{l r r}
	\toprule
	\textbf{Statistics}							   &	\textbf{\#}	& 	\textbf{\%}	\\
	\midrule
	All projects analyzed			&	489		&	100.00		\\
	Projects with suspicious unsafe usage				  
												& 52		  & 10.6			\\
	
	\bottomrule
\end{tabular}

==> tables/rq3-top10-unsafe-badpractices.tex <==
\begin{tabular}{lr}
\toprule
\multirow{2}{*}{\textbf{Project}}          &  \textbf{\# of reported risky}\\
					& \textbf{pointer conversion}	\\
\midrule
cznic/sqlite     &  6496 \\
xlab/android-go  &   270 \\
gotk3/gotk3      &   267 \\
conformal/gotk3  &   159 \\
vulkan-go/vulkan &   134 \\
uber/aresdb      &    46 \\
go-qml/qml       &    37 \\
atmanos/atmanos  &    32 \\
lxn/walk         &    24 \\
go-gl/gl         &    19 \\
\bottomrule
\end{tabular}
